Feasible Region: an Actuation-Aware Extension of the Support Region

In legged locomotion the projection of the robot Center of Mass (CoM) being inside the convex hull of the contact points is a commonly accepted sufficient condition to achieve static balancing. However, some of these configurations cannot be realized because the joint torques required to sustain them would be above their limits (actuation limits). In this manuscript we rule out such configurations and define the Feasible Region, a revisited support region that guarantees both global static stability in the sense of tipover and slippage avoidance and of existence of a set of joint-torques that are able to sustain the robot body weight. We show that the feasible region can be employed for the selection of feasible footholds and CoM trajectories to achieve static locomotion on rough terrains, also in presence of load intensive tasks. Key results of our approach include the efficiency in the computation of the feasible region thanks to an Iterative Projection algorithm. This allowed us to carry out successful experiments on the HyQ robot, that was able to negotiate obstacles of moderate dimensions while carrying an extra 10 kg payload.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/global_region.tex <==
\section{The Global Actuation and Feasible Regions}\label{sec:globalRegion}
	In this Section we address the issues due to the configuration dependency of the local feasible region and propose a \textit{global} extension that is not configuration dependent and only depends on joint-torque limits and the location of contact points.\\
	Figure~\ref{fig:variableCoMActuationRegions} shows the local feasible region computed for different \gls{CoM} positions (along the same segment from $(0,-0.3)$ to $(0,+0.3)$) and for the same set of contact points. As previously anticipated, the local feasible regions $\mathcal{Y}_{fa}$ change as a function of the robot's configuration while the friction region $\mathcal{Y}_{f}$ (dashed blue line) is constant as it only depends on the stance locations and orientation.
	\begin{figure}
		\centering	
		\includegraphics[width=9cm]{figs/actuation_region/instantaneous_actuation_region_variable_com2}
		\caption[Local actuation areas for different CoM positions]{Local actuation areas for the same foothold positions and for different \gls{CoM} positions along the same segment. The triangular markers represent those \gls{CoM} positions that do not belong to their correspondent local feasible region. The squared markers, instead, represent the tested \gls{CoM} positions that are inside their correspondent local feasible region.}
		\label{fig:variableCoMActuationRegions}
	\end{figure}
	
	By inspection of the resulting actuation areas $\mathcal{Y}_{a}$ is evident that some of the \gls{CoM} positions $\vc{c}_{xy}$ used for their computation do not lie within their corresponding local actuation region; such points are marked with squared markers. This is a degenerate condition in which the set of feasible forces/wrenches (constrained by the  wrench polytopes and thus, ultimately, depending on the limb Jacobians $\vc{J}_i$ and on the torque limits $\vc{\tau}^{lim}_i$) are not able to withstand the weight of the robot lumped into the specified value of $\vc{c}_{xy}$. Those cases are therefore to be considered unfeasible, even if the area of the resulting local actuation region is not empty. Such degenerate areas might be useful in the unlikely cases where the \gls{CoM} position $\vc{c}_{xy}$ changes without changing the robot configuration (\eg when an external static load is added onto the trunk of the robot at a decentralized location).\\
	Those points that \emph{do} belong to their respective local actuation region are instead marked with triangular markers.\\
	By repeating the test shown in Fig. \ref{fig:variableCoMActuationRegions} along multiple directions and with multiple $\vc{c}_{xy}$ positions (and, consequently different robot configurations) one can notice that the set of feasible \gls{CoM} positions results in a convex set that we name the \textit{global actuation region} $\mathcal{G}_a$:
	
	\textbf{Definition 1:} the static \textit{global actuation region} $\mathcal{G}_a$ is the set of all \gls{CoM} coordinates $\vc{c}_{xy} \in \Rnum^2$, lying on the plane orthogonal to the direction of gravity, where the robot is able to withstand its own weight considering its own joint-kinematic and joint-torque limits. 
	
	The definition above does not include the unilaterality of contact forces nor friction constraints; we thus define as follows a second global region that also considers such features (see Tab.~\ref{tab:2}).
	
	\textbf{Definition 2:} the static \textit{global feasible region} $\mathcal{G}_{fa}$ is the set of all \gls{CoM} coordinates $\vc{c}_{xy} \in \Rnum^2$, orthogonal to the direction of gravity, where the robot is able to withstand its own weight, considering its own kinematics, its joint-torque limits, the unilaterality of contact forces and the friction constraints. 

	\begin{table}[!b]
		\label{tab:vertexBasedProjectionAlgorithm}
		\begin{center}
			\begin{tabular}{ | c | c | c|}
				\hline
				constraint &  2D \gls{CoM} space & validity \\ \hline
				friction   & friction/support region $\mathcal{Y}_f$  &  global\\
				joint-torques    & actuation region $\mathcal{Y}_a$  & local\\
				friction  $\&$ joint-torques    & feasible region $\mathcal{Y}_{fa}$ & local \\
				joint-torques    & actuation region $\mathcal{G}_a$ & global\\
				friction $\&$ joint-torques    & feasible region $\mathcal{G}_{fa}$  & global\\
				\hline
			\end{tabular}
			\caption{Summary about the local/global validity of feasible regions.}
            \label{tab:2}
		\end{center}
	\end{table}
	
The two areas $\mathcal{G}_a$ and $\mathcal{G}_{fa}$, unlike their local counterparts $\mathcal{Y}_a$ and $\mathcal{Y}_{fa}$, are \textit{independent} from the robot configuration and they only depend on contact locations. \\
	\begin{figure}
		\centering
		\begin{subfigure}{4.5cm}
			\includegraphics[width=1\textwidth]{figs/actuation_region/local_region_grid_points}
			\caption{Grid sampling and rectangular cells partitioning.}
			\label{fig:local_region_grid_points}
		\end{subfigure}
		~
		\begin{subfigure}{4cm}
			\includegraphics[width=1\textwidth]{figs/actuation_region/local_region_random_uniform_points}
			\caption{Random uniform sampling with Voronoi tessellation.}
			\label{fig:local_region_random_uniform_points}
		\end{subfigure}
		
		\captionsetup{singlelinecheck=off}
		\caption[Global feasible region for the JVRC-1 humanoid robot]{Friction region (green) and global feasible region (blue) for the JVRC-1 humanoid robot.}
		\label{fig:humanoidRegion}
	\end{figure}
	Figure~\ref{fig:humanoidRegion} shows the global feasible area $\mathcal{G}_{fa}$ (blue area) and the friction region $\mathcal{Y}_{f}$ (green area) for the Japan Virtual Robotics Challenge (JVRC-1) humanoid robot \cite{diankov_thesis2010}. The blue region $\mathcal{G}_{fa}$ in Fig. \ref{fig:local_region_grid_points} was obtained by consecutively computing the local actuation areas over a two-dimensional grid of points with a predefined resolution. Considering that, by construction, the global feasible area $\mathcal{G}_{fa}$ must be included inside the friction region $\mathcal{Y}_{f}$ (green), grid points were only generated inside $\mathcal{Y}_{f}$.\\
	The red (resp. green) dots in Fig.~\ref{fig:humanoidRegion} correspond to those \gls{CoM} locations that do not (resp. do) belong to their own local feasible region. For a green grid point, we intersect the local actuation region with a small rectangle of grid dimensions so as to enforce the fact that the local actuation region is only valid in a small neighborhood of the corresponding grid point. The global feasible region (dark green line) $\mathcal{G}_{fa}$ is then obtained as the convex hull of all local blue regions. One can observe that some grid points that should be inside $\mathcal{G}_{fa}$ are actually red because of numerical artifacts close to the boundaries.
	
	The explained strategy yields the desired global actuation region $\mathcal{G}_{fa}$, however, the computation is not efficient (a new \gls{IP} problem has to be solved at every grid point) and its accuracy depends on the predefined resolution of the grid map. We propose a more efficient strategy based on uniform random sampling and the use of Voronoi tessellation, as shown in Fig. \ref{fig:local_region_random_uniform_points}. 
	The partition is generated starting from a uniform distribution of $n$ sample points in a convex set (in this case inside $\mathcal{Y}_{f}$). Recall that using a uniform distribution to generation a Voronoi diagram minimizes the variance of the areas of each individual Voronoi cells. By intersecting local actuation regions with the Voronoi cell of their sample point, we can compute the same area $\mathcal{G}_{fa}$ as previously, yet with a sample size that is less than half of the initial strategy.
	
	\subsection{Sequential Iterative Projection (SIP) Algorithm}\label{sec:sip}
	In this Section we present an alternative to the previous sampling-based approaches for the computation of the global feasible region. This consists of a recursive solution of the \gls{IP} algorithm presented in Section \ref{sec:localActuationRegion} (Alg. \ref{alg:iterativeProjectionWithActuation}).
	The algorithm is based on the observation that, if the same set of contacts is kept, varying the robot configurations will result in one of the two following events:
	\begin{enumerate}
		\item  $\mathcal{Y}_{fa}$ degenerates to an empty area (either because the Jacobian matrix $\vc{J}_i$, used for the computation of $\vc{G}$ in ~\eqref{eq:actuationInequalities}, becomes singular or because torque limits are exceeded);
		\item $\mathcal{Y}_{fa}$ has a positive area but the projection of the \gls{CoM} is not inside it (as mentioned in Sec. \ref{sec:globalRegion}).
	\end{enumerate}
	Case 1) occurs most commonly when the robot's load increases beyond the maximum value allowed by the joint-torque limits. If, instead, the robot's mass is constant (no external loads and/or disturbances) then the event 2) usually occurs before event 1).\\
	Based on this observation, starting from a default \gls{CoM} position we update the robot's configuration while we move the \gls{CoM} along a desired direction,  represented by the unit vector $\vc{a} \in \Rnum^2$, and sequentially recompute the instantaneous actuation region (using Alg. \ref{alg:iterativeProjectionWithActuation}) until the distance between the edges of $\mathcal{Y}_{fa}$ and the \gls{CoM} projection becomes smaller than the predefined acceptable tolerance $\epsilon$ (see Alg. \ref{alg:sip}).
	
			\begin{algorithm}
				\textbf{Input: }{$\vc{c}, \vc{p}_1, \dots, \vc{p}_{n_c}, \vc{n}_1, \dots ,\vc{n}_{n_c}, \mu_1, \dots, \mu_{n_c}, \vc{g}_1, \dots, \vc{g}_{n_c},$}\; {$\vc{J}_1, \dots, \vc{J}_{n_c}, \vc{\tau}^{lim}_1, \dots ,\vc{\tau}^{lim}_{n_c}$}\;
				\KwResult {vertex $\hat{\vc{c}}$ of the global feasible region $\mathcal{G}_{fa}$ along the direction $\vc{a}\in \Rnum^2$}
				Initialization: {set the initial vertex guess $\hat{\vc{c}} \in \Rnum^2$ equal to the default \gls{CoM} ($x,y$) coordinates: $\hat{\vc{c}}_0 = P \vc{c}$}\;
				Set $d = \infty$ and $\epsilon \rightarrow 0$\;
				\While{$d > \epsilon$}{
					I) compute the contact points $\vc{p}^{\hat{\vc{c}}}_{1}, \dots, \vc{p}^{\hat{\vc{c}}}_{n_c}$ in the new \gls{CoM} frame located in $\hat{\vc{c}}_i$\;
					II) solve inverse kinematics: $\vc{q} = IK(\vc{p}^{\hat{\vc{c}}}_{1}, \dots \vc{p}^{\hat{\vc{c}}}_{n_c})$\;
					III) compute $\vc{G}$ and $\vc{d}$ as in ~\eqref{eq:actuationInequalities} for the joint configuration $\vc{q}$\;
					IV) $\mathcal{Y}_{fa} = IP(\vc{A}_1, \vc{A}_2, \vc{B}, \vc{u}, \vc{G},\vc{d})$\;
					V) find the intersection $\vc{e} \in \Rnum^2$ between the desired direction $\vc{a}$ and the edges of $\mathcal{Y}_{fa}$\;
					VI) $d = ||\vc{e} - \hat{\vc{c}}||_2$\;
					VII) update the vertex $\hat{\vc{c}}$ towards $\vc{e}$: $\hat{\vc{c}}_{k+1} = \hat{\vc{c}}_k + \alpha (\vc{e} - \hat{\vc{c}}_k)$
				}
				%\end{algorithm}
				
				\caption{Sequential Iterative Projection (SIP) Algorithm}
				\label{alg:sip}
			\end{algorithm}

	
	{In contrast to} the tests reported in Fig. \ref{fig:variableCoMActuationRegions} (where all the \gls{CoM} were homogeneously distributed along one segment), in this case we increasingly update the new tested \gls{CoM} position $\hat{\vc{c}}$ of a given gain $\alpha$ of the distance $d$ between the current value of the \gls{CoM} position and the intersection $\vc{e}$ between the local region $\mathcal{Y}_{fa}$ and the considered search direction:
	\begin{equation}
	d = ||\vc{e} - \hat{\vc{c}}||_2
	\end{equation}
	With the usage of a suitable gain $\alpha$, this allows the distance $d$ to recursively converge to zero; whenever the distance becomes lower than the predefined tolerance $\epsilon$ the procedure is stopped and the latest \gls{CoM} position $\hat{\vc{c}}$ is considered to be a vertex of the global feasible region $\mathcal{G}_{fa}$.
	
	This strategy allows one to efficiently find a vertex on the edge of the global feasible region by recursive computations of the \gls{IP} algorithm. The strategy can then be repeated in multiple directions (see for example Fig. \ref{fig:sip}b) in order to reconstruct the entire global feasible region $\mathcal{G}_{fa}$ or just a part of it in the region of most interest.
	
	\begin{figure}
			\centering
			\begin{subfigure}{4.2cm}
				\includegraphics[width=0.9\textwidth]{figs/actuation_region/newSequentialIterativeProjection}
				\caption{Convergence of the distance $d_i = ||\vc{e}_i - \hat{\vc{c}}_i||_2$ along a given search direction.}
				\label{fig:sip1}
			\end{subfigure}
			~
			\begin{subfigure}{4.2cm}
				\includegraphics[width=0.9\textwidth]{figs/actuation_region/newSequentialIterativeProjection2}
				\caption{Repetition of the SIP algorithm along different search directions}
				\label{fig:sip2}
			\end{subfigure}
			\captionsetup{singlelinecheck=off}
			\caption{Visual representation of the estimation of the global feasible region using the SIP algorithm.}
			\label{fig:sip}
		\end{figure}
		
	The underlying idea of the \gls{SIP} algorithm (\ie to sequentially change one quantity (\gls{CoM} position, trunk orientation or feet positions) and to-recompute a new local area till when the convergence criterion is met) remains therefore valid.
	
	The global feasible region $\mathcal{G}_{fa}$ as defined so far is independent from the robot's $(x,y)$ coordinates; however, it still depends on the robot's height and trunk orientation. In the next Section we will attempt to exploit the dependency of $\mathcal{G}_{fa}$ from the robot's height ($z$ coordinate) in order to estimate a 3D volume of friction- and actuation-consistent \gls{CoM} positions.
	
	\subsection{3D Global Feasible Volume}\label{sec:feasibleVolume}
	Fig. \ref{fig:ladder_climb} depicts the JVRC-1 robot climbing a vertical ladder. In this case, we model the robot with unilateral contact constraints (intersection of friction cones and wrench polytopes) at the feet and bilateral contacts (only wrench polytopes and no friction cone constraints) at the hands. We then compute the friction region $\mathcal{Y}_{f}$ using Alg. \ref{alg:iterativeProjectionBretl} setting infinite values of the friction coefficient on hand contacts. This yields as a result the whole horizontal plane as friction region. This is due to the fact that, because of the opposition of the contacts on the vertical ladder, the robot is able to exert any contact force, so it could ideally locate its \gls{CoM} anywhere in the $x,y$ plane (if kinematic limits are not considered). 
	
	The blue convex set in Fig. \ref{fig:3D_actuation_volume_sliced} is the global feasible region $\mathcal{G}_{fa}$. The blue 3D volume in Fig. \ref{fig:3D_actuation_volume} is the convex hull of multiple $\mathcal{G}_{fa}$ computed at different robot heights.  $\mathcal{G}_{fa}$ can therefore be seen as a \textit{slice} of the blue 3D volume in the direction orthogonal to gravity.\\
	In the ladder climbing scenario, the robot-specific kinematics highly affect the climbing capabilities of the robot. This can be captured by the upper and lower bounds of the 3D feasible volume which, depending on the values of the torque limits, may be due to either of two following causes:
	\begin{enumerate}
		\item the area of the 2D global feasible region $\mathcal{G}_{fa}$ converging to zero. This condition is due to the magnitude of the actuation limits which is too low to carry the body weight for that configuration;
		\item the arms or legs' Jacobians reaching a kinematic singularity (\ie point 1 in Section \ref{sec:sip}). This is due to a degeneration of the wrench polytopes, regardless the value of the actuation limits.
	\end{enumerate}
	The usage of 3D feasible volumes, such as the one shown in this picture, could overcome the typical limitation of static equilibrium approaches for which the \gls{CoM} height $c_z$ is unobservable (because parallel to gravity). Such 3D volumes could indeed enable the planning of friction- and actuation-consistent robot height trajectories (besides the planning of the coordinates orthogonal to gravity) at the price of larger computation times.

\begin{figure}
		\centering
		\begin{subfigure}{4cm}
			\includegraphics[width=0.9\textwidth]{figs/actuation_region/ladder_climb1}
			\caption{Friction region (green) and global feasible region (blue) for a specific robot height.}
			\label{fig:3D_actuation_volume_sliced}
		\end{subfigure}
		~
		\begin{subfigure}{4cm}
			\includegraphics[width=0.9\textwidth]{figs/actuation_region/ladder_climb_frame}
			\caption{Friction region (green) and global feasible volume (blue)}
			\label{fig:3D_actuation_volume}
		\end{subfigure}
		\captionsetup{singlelinecheck=off}
		\caption[JVRC-1 humanoid robot climbing a ladder]{JVRC-1 humanoid robot climbing a ladder.}
		\label{fig:ladder_climb}
	\end{figure}
